Spoofed training data for speech spoofing countermeasure can be efficiently created using neural vocoders

A good training set for speech spoofing countermeasures requires diverse TTS and VC spoofing attacks, but generating TTS and VC spoofed trials for a target speaker may be technically demanding. Instead of using full-fledged TTS and VC systems, this study uses neural-network-based vocoders to do copy-synthesis on bona fide utterances. The output data can be used as spoofed data. To make better use of pairs of bona fide and spoofed data, this study introduces a contrastive feature loss that can be plugged into the standard training criterion. On the basis of the bona fide trials from the ASVspoof 2019 logical access training set, this study empirically compared a few training sets created in the proposed manner using a few neural non-autoregressive vocoders. Results on multiple test sets suggest good practices such as fine-tuning neural vocoders using bona fide data from the target domain. The results also demonstrated the effectiveness of the contrastive feature loss. Combining the best practices, the trained CM achieved overall competitive performance. Its EERs on the ASVspoof 2021 hidden subsets also outperformed the top-1 challenge submission.

==> app_tab1.tex <==

\begin{table}[!h]
\centering
\Large
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.5}
\caption{Results of statistical significance analysis for EERs in Table~\ref{tab:exp-1} (Part 1). Grey block indicates statistical significant difference.}
\resizebox{0.7\columnwidth}{!}
{
\begin{tabular}{cccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 {\setELA}                               &  \multicolumn{3}{c}{\rotatebox{90}{\setTLAshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTWFshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTVIshort}}  & \multicolumn{3}{c}{\rotatebox{90}{\setTVIIIshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTVIVshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}}  \\ 
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
 {\setELAII}                             \\ 
 \midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
 {\setEDF}                             \\ 
 \midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\end{tabular}
\label{tab:app-sig-1}
}
\end{table}


\begin{table}[!h]
\centering
\caption{Results of statistical significance analysis for EERs in Table~\ref{tab:exp-1} (Part 2). Grey block indicates statistical significant difference.}
\Large
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.5}
\resizebox{0.7\columnwidth}{!}
{
\begin{tabular}{cccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 {\setELATRIM}                               &  \multicolumn{3}{c}{\rotatebox{90}{\setTLAshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTWFshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTVIshort}}  & \multicolumn{3}{c}{\rotatebox{90}{\setTVIIIshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTVIVshort}}  &  \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}}  \\ 
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
{\setELAHID} \\
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
\setEDFHID \\
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
\setEWFE \\
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\\
\setEDFE \\
\midrule
 \multirow{3}{*}{\setTLAshort}  &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTWFshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVIshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIIIshort} &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
\multirow{3}{*}{\setTVIVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
\hline
 \multirow{3}{*}{\setTVVshort}  &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}         \\ 
                                &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{0.59, 0.59, 0.59}          &         \cellcolor[rgb]{1.00, 1.00, 1.00}         \\ 
\bottomrule
\end{tabular}
}
\label{tab:app-sig-2}
\end{table}





==> app_tab2.tex <==

\begin{table}[!h]
\centering
\caption{Results of statistical significance analysis for EERs in Table~\ref{tab:exp-2} (Part 1). Grey block indicates statistical significant difference.}
\Huge
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{0.6}
\resizebox{0.70\columnwidth}{!}
{
\begin{tabular}{cccc|ccc|ccc|ccc|ccc|ccc|ccc}

     \multicolumn{1}{l}{Training criterion}  & \multicolumn{12}{c}{$\mathcal{L}_{\text{CE}}$ }   & \multicolumn{9}{c}{$\mathcal{L}_{\text{CE}} + \mathcal{L}_{\text{CF}}$ }   \\
  \cmidrule(lr){2-13}\cmidrule(lr){14-22} 
    \multicolumn{1}{l}{Data augmentation} &  \multicolumn{6}{c}{$\times$} & \multicolumn{15}{c}{RawBoost}  \\
  \cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-22} 
    \multicolumn{1}{l}{Training set}     &  \multicolumn{3}{c}{\rotatebox{90}{\setTLAshort}}    & \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTLAshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTLAshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}} & \multicolumn{3}{c}{\rotatebox{90}{\setTVVshort}}\\ 
  \multicolumn{1}{l}{Bona-spoof paired}   &  \multicolumn{3}{c}{$\times$}  &  \multicolumn{3}{c}{$\times$}  &  \multicolumn{3}{c}{$\times$}  &  \multicolumn{3}{c}{$\times$}  &  \multicolumn{3}{c}{$\times$}  &  \multicolumn{3}{c}{$\times$} &  \multicolumn{3}{c}{$\checkmark$} \\
\toprule
 {\setELA}  & \multicolumn{3}{c}{\selfcircle{1}} & \multicolumn{3}{c}{\selfcircle{2}} & \multicolumn{3}{c}{\selfcircle{3}} & \multicolumn{3}{c}{\selfcircle{4}} & \multicolumn{3}{c}{\selfcircle{5}} & \multicolumn{3}{c}{\selfcircle{6}} & \multicolumn{3}{c}{\selfcircle{7}}    \\ 
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
 {\setELAII}                     \\
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
            & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
{\setEDF}                \\
\midrule 
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
           & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\end{tabular}
}
\label{tab:app-sig-3}
\end{table}




\begin{table}[!h]
\centering
\caption{Results of statistical significance analysis for EERs in Table~\ref{tab:exp-2} (Part 2). Grey block indicates statistical significant difference.}
\Huge
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{0.6}
\resizebox{0.70\columnwidth}{!}
{
\begin{tabular}{cccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 {\setELATRIM}               & \multicolumn{3}{c}{\selfcircle{1}} & \multicolumn{3}{c}{\selfcircle{2}} & \multicolumn{3}{c}{\selfcircle{3}} & \multicolumn{3}{c}{\selfcircle{4}} & \multicolumn{3}{c}{\selfcircle{5}} & \multicolumn{3}{c}{\selfcircle{6}} & \multicolumn{3}{c}{\selfcircle{7}}    \\ 
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
{\setELAHID} \\
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
\setEDFHID \\
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
\setEWFE \\
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\\
\setEDFE \\
\midrule
\multirow{3}{*}{\selfcircle{1}} & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{2}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{3}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{4}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{5}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
\hline
\multirow{3}{*}{\selfcircle{6}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\hline
\multirow{3}{*}{\selfcircle{7}} & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59} \\ 
                                & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{1.00, 1.00, 1.00}  & \cellcolor[rgb]{0.59, 0.59, 0.59}  & \cellcolor[rgb]{1.00, 1.00, 1.00} \\ 
\bottomrule
\end{tabular}
}
\label{tab:app-sig-4}
\end{table}



